Multi-agent Bayesian Learning with Best Response Dynamics: Convergence and Stability

We study learning dynamics induced by strategic agents who repeatedly play a game with an unknown payoff-relevant parameter. In this dynamics, a belief estimate of the parameter is repeatedly updated given players' strategies and realized payoffs using Bayes's rule. Players adjust their strategies by accounting for best response strategies given the belief. We show that, with probability 1, beliefs and strategies converge to a fixed point, where the belief consistently estimates the payoff distribution for the strategy, and the strategy is an equilibrium corresponding to the belief. However, learning may not always identify the unknown parameter because the belief estimate relies on the game outcomes that are endogenously generated by players' strategies. We obtain sufficient and necessary conditions, under which learning leads to a globally stable fixed point that is a complete information Nash equilibrium. We also provide sufficient conditions that guarantee local stability of fixed point beliefs and strategies.

==> adaptive_learning.tex <==
% !TEX root = main041620.tex
%%novalidate
\section{Learning with Best-response Strategies}\label{sec:br}
In Sec. \ref{subsec:results_br}, we derive convergence and stability results for learning with best-response strategies \eqref{eq:update_belief} -- \eqref{eq:eq_update} under certain assumptions of stepsizes and best response correspondence. In Sec. \ref{subsec:two_class}, we show that these assumptions hold in two classes of games -- potential games and dominance solvable games. 

\subsection{Convergence and Stability Analysis}\label{subsec:results_br}
Since belief is updated as in \eqref{eq:update_belief}, analogous to Lemma \ref{lemma:theta_eq}, the beliefs converge to a fixed point belief $\thetabar$ with probability 1. However, in contrast to \eqref{eq:eq_update}, the best response strategy profile $\gbr(\thetatone, \qt)=\(\gibr(\thetatone, \qt_{\mi})\)_{\i \in \I}$ in \eqref{eq:br_update} depends on the updated belief $\thetatone$ as well as the current strategy profile $\qt$. Hence, the strategy profile in each step can no longer be expressed as a linear combination of the initial strategy and continuous functions of beliefs. Therefore, the approach of proving the convergence of strategies in Lemma \ref{lemma:q_eq} does not apply to learning with best response strategies. We now develop a new approach to analyze the convergence of $\qt$ for \eqref{eq:br_update}.





Based on Lemma \ref{lemma:theta_eq}, we consider any sequence of beliefs $\(\thetat\)_{\t=1}^{\infty}$ that converges to a fixed point belief $\thetabar$. In each step $\t$ with the belief $\theta^{\t+1}$, for any best response strategy $\gibr(\thetatone, \qt_{\mi}) \in \BRi\(\theta^{\t+1}, \qt_{\mi}\)$ in the strategy update \eqref{eq:br_update}, we can find another strategy $\tilde{h}_\i(\thetabar, \qt_{\mi})$ in the best response correspondence $\BRi(\thetabar, \qt_{\mi})$ with respect to the fixed point belief $\thetabar$ such that the distance between $\tilde{h}_\i(\thetabar, \qt_{\mi})$ and $\gibr(\thetatone, \qt_{\mi})$ attains a minimum, i.e. $\tilde{h}_\i(\thetabar, \qt_{\mi})= \argmin_{\qi \in \BRi(\thetabar, \qt_{\mi})} $ $|\qi-\gibr(\thetatone, \qt_{\mi})|$. We define $\xi_i^{\t}\deleq \gibr(\thetatone, \qt_{\mi})-\tilde{h}_\i(\thetabar, \qt_{\mi})$. Then, the strategy update \eqref{eq:br_update} in each step $\t$ can be re-written as follows: 
\begin{align}\label{eq:rewrite_dynamics}
    \q^{\t+1}_i  -\qit&=\ait \(\gibr(\thetatone, \qt_{\mi})-\qit\)= \ait\(\tilde{h}_\i(\thetabar, \qt_{\mi})-\qit+\xi_i^{\t}\).
\end{align}
We define the maximum stepsize in step $\t$ as $\bar{a}^\t=\max_{\i \in \I} \ait$, and assume that the ratio between the stepsizes of all players and the maximum stepsize are lower bounded by a positive number: 

\textbf{(A3)} $\frac{\ait}{\bar{a}^\t} \geq \nu>0$ for all $\i \in \I$ and all $\t$.

Then, since $\tilde{h}_\i(\thetabar, \qt_{\mi}) \in \BRi(\thetabar, \qt_{\mi})$ for all $\i \in \I$ and all $\t$, we can write \eqref{eq:rewrite_dynamics} as a discrete-time asynchronous best response dynamics for the game $\G$ with the fixed point belief $\thetabar$ and residual terms $\xi^{\t}= \(\xi^{\t}_i\)_{i \in \I}$: 
\begin{align}\label{eq:discrete}
    \q^{\t+1} -\qt \in \bar{a}^\t \mathcal{A}\cdot \(\BR\(\thetabar, \qt\) - 
    \qt + \xi^{\t}\),
\end{align}
where $\mathcal{A} \cdot\(\BR\(\thetabar, \qt\)-\qt+ \xi^{\t}\) \deleq \left\{A \cdot \(\tilde{h}(\thetabar, \qt)-\qt+ \xi^{\t}\) \left\vert A \in \mathcal{A}, ~ \tilde{h}(\thetabar, \qt) \in \BR(\thetabar, \qt) \right. \right\}$, and
\begin{align}
    \mathcal{A} \deleq \left\{A \in \mathbb{R}^{dim(\Q)\times dim(\Q)}\left\vert
     \begin{array}{l}
     A=diag(\underbrace{\alpha_1 \dots \alpha_1}_{dim\(\Q_1\)}, \dots, \underbrace{\alpha_i \dots \alpha_i}_{dim\(\Qi\)} , \dots, \underbrace{\alpha_I \dots \alpha_I}_{dim\(Q_I\)}).\\
     \alpha_i \in [\nu, 1], \quad \forall \i \in \I
    \end{array}\right.\right\}.\label{subeq:Lambda}
\end{align}
The diagonal matrix $A \in \mathcal{A}$ in \eqref{subeq:Lambda} captures the asynchronous nature of players' strategy updates, with $\alpha_i$ denoting the ratio between the stepsize of player $\i \in \I$ and the maximum stepsize in step $\t$. From Assumption \textbf{(A3)}, we know that each diagonal value $\alpha_i$ is lower bounded by $\nu$ for all $\i \in \I$. If the step sizes of all players are identical (i.e. $\ait=\at_{j}$ for all $i, j \in \I$ and all $\t$), then the best response dynamics is synchronous and the matrix $A$ is an identity matrix. 



We apply the theory of stochastic approximation to show the convergence of strategies in \eqref{eq:discrete}; see \cite{borkar1998asynchronous}, \cite{benaim2005stochastic}, \cite{benaim2006stochastic}, and \cite{perkins2013asynchronous}. The theory allows us to analyze the asymptotic properties of the strategy sequence $\(\qt\)_{\t=1}^{\infty}$ by approximating the discrete-time dynamics \eqref{eq:discrete} with a continuous time best-response differential inclusion given by: 
\begin{align}\label{eq:differential_inclusion}
    \frac{d \qdiff(\tau)}{d \tau} \in \mathcal{A} \cdot \(\BR\(\thetabar, \qdiff\)-\qdiff\)
\end{align}
where $\mathcal{A} \cdot\(\BR\(\thetabar, \qdiff\)-\qdiff\) \deleq \left\{A \cdot \(\tilde{\gbr}(\thetabar, \qdiff)-\qdiff\) \left\vert A \in \mathcal{A}, ~ \tilde{\gbr}(\thetabar, \qdiff) \in \BR(\thetabar, \qdiff) \right. \right\}$ and $\mathcal{A}$ is defined as in \eqref{subeq:Lambda}.
A solution of \eqref{eq:differential_inclusion} with the initial strategy profile $\q^1 \in \Q$ is an absolutely continuous function $\tilde{\q}(\tau): [1, \infty) \to \Q$ such that $\tilde{\q}(1)=\q^1$, and $\tilde{\q}(\tau)$ satisfies \eqref{eq:differential_inclusion} for almost all $\tau \geq 1$. We adopt the assumptions from \cite{perkins2013asynchronous} for asynchronous best response dynamics: 




\textbf{(A4)} For each $\t$, the maximum stepsizes $\(\atbar\)_{\t=1}^{\infty}$ satisfy the following conditions: 
\begin{equation*}%\label{eq:stepsize}
\begin{split}
    \sum_{\t=1}^{\infty} \atbar &=\infty, \quad 
    \sum_{\t=1}^{\infty} \(\atbar\)^2 < \infty, \quad 
    \atbar \geq \abar^{\t+1}, \quad \forall \t, \\% \label{subeq:step_size_br}\\
    \sup_{\t} \frac{\abar^{\lfloor x\t \rfloor}}{\atbar} &< \infty, \quad \forall x \in (0, 1], %\label{subeq:x}
\end{split}
\end{equation*}
where $\lfloor x\t \rfloor$ is the largest integer that is smaller than $x\t$. 




\textbf{(A5)} For any $\theta \in \Delta(\S)$ and any $\qmi \in \Q_{\mi}$, the best response correspondence $\BRi(\theta, \qmi)$ is a convex and compact set in $\Q$. Additionally, $\BRi(\theta, \qmi)$ is upper-hemicontinuous in both $\theta$ and $\qmi$ for all $\i \in \I$.


\textbf{(A6)} For any $\theta \in \Delta(\S)$ and any $\q^1 \in \Q$, any solution $\qdiff(\tau)$ of \eqref{eq:differential_inclusion} such that $\qdiff(1)=\q^1$ satisfies $\lim_{\tau \to \infty} \mathrm{dist}\(\qdiff(\tau), \EQ(\theta)\)=0$.


Assumption \textbf{(A4)} is a standard requirement on step sizes in stochastic approximation \cite{borkar2009stochastic}. Assumption \textbf{(A5)} ensures that the solutions of the differential inclusion \eqref{eq:differential_inclusion} exist given any initial strategy $\q^1 \in \Q$. Assumption \textbf{(A6)} requires that given any initial strategy $\q^1 \in \Q$, the continuous-time best response dynamics converges to the equilibrium set of the game $\G$ for any constant belief $\theta$. 

Not all games satisfy \textbf{(A5)} -- \textbf{(A6)}. For example, best response dynamics is cyclic in the well-known generalized rock-paper-scissors game with complete information so \textbf{(A6)} is not satisfied by this game, see \cite{shapley1964some}. In Sec. \ref{subsec:two_class}, we demonstrate that \textbf{(A5)} -- \textbf{(A6)} are guaranteed in two classes of games -- potential games and dominance solvable games. 



Based on \textbf{(A3)} -- \textbf{(A6)}, we have the following:

\begin{theorem}\label{prop:asynchronous}
For any initial state~$(\theta^1, \q^1) \in \Delta(\S) \times \Q$, under assumptions \textbf{(A3)} -- \textbf{(A6)}, the sequence of states $(\thetat, \qt)_{\t=1}^{\infty}$ generated by the learning dynamics~\eqref{eq:update_belief} and \eqref{eq:br_update} satisfy $\lim_{\t \to \infty} \thetat =\thetabar$ and $\lim_{\t \to \infty} \mathrm{dist}\(\qt, \EQ(\thetabar)\)=0$ with probability 1. 

Moreover, the belief $\thetabar$ satisfies $[\thetabar] \subseteq \Sequiv(\limitq)$ with probability 1, where $\limitq \subseteq \EQ(\thetabar)$ is the limit set of the strategy sequence $\(\qt\)_{\t=1}^{\infty}$. 
\end{theorem}





Analogous to Theorem \ref{theorem:convergence_eq}, this result ensures that in learning with best response strategies, the convergent belief $\thetabar$ accurately estimates the payoff distribution given players' strategies, and players eventually play equilibrium strategies in game $\G$ with belief $\thetabar$. 

We now provide a set of sufficient conditions that guarantee local stability of $\(\thetabar, \EQ(\thetabar)\)$ for learning with best response strategies. The global stability property is identical to that of the learning dynamics with equilibrium strategies, as stated in Proposition \ref{prop:global}.  

\begin{theorem}\label{theorem:stability_br}
A fixed point belief $\bar\theta\in\Delta(S)$ and the corresponding equilibrium set $EQ(\bar\theta)$ is locally stable under the learning dynamics \eqref{eq:update_belief}
and \eqref{eq:br_update} if Assumptions \textbf{(A3)} -- \textbf{(A6)} are satisfied, and the following conditions hold: (a) $EQ(\theta)$ is upper-hemicontinuous in $\theta$;
(b) 
\end{theorem}
Condition {\em (a)} in Theorem \ref{theorem:stability_br} is the same as that in Theorem \ref{theorem:stability_eq}. This condition ensures that if the convergent belief is close to $\thetabar$, then the convergent strategy will also be close to $\EQ(\thetabar)$. Condition {\em (b)} in Theorem \ref{theorem:stability_br} is more restrictive than in Theorem \ref{theorem:stability_eq} -- it not only ensures that all parameters in $[\thetabar]$ are payoff-equivalent (given any strategy) in a local neighborhood of $\EQ(\thetabar)$, but also requires that the best response strategy profile $\gbr(\theta, \q)$ remains close to the set $\EQ(\thetabar)$ when $\q$ and $\theta$ are locally perturbed in a small neighborhood of $\EQ(\thetabar)$ and $\thetabar$, respectively. These two conditions together guarantee local stability. The proof builds on Theorem \ref{theorem:stability_br}, and is included in Appendix \ref{apx:proof}. 









==> belief_converge.tex <==
%%novalidate
\section{Empirical Consistency of Belief Update}

We make the following two assumptions: 

\emph{\textbf{(A1)} The probability density function $\phibar^\s(\cbar|\q)$ is continuous in $\q$ for all $\s \in \S$. }

\emph{\textbf{(A2)} 
$\theta^1(\s)>0$ for all $\s \in \S$.}

The estimated distribution of payoff given $\theta$ and $\q$ is given by: 
\begin{align*}
    \mutheta\(\c|\q\) = \sum_{\s \in \S} \theta(\s) \phi^\s(\c|\q). 
\end{align*}


\begin{definition}[Distinguishable parameters]\label{def:observe}
For any strategy profile $\q\in \Q$, parameter $s$ is distinguishable from the true parameter $\sran$ based on the realized outcome $\cbar$ if the Kullback–Leibler (KL) divergence from the distributions of $\cbar$ with $\s$ to the distribution with $\sran$ is positive, i.e.
\begin{align}\label{eq:KL_distinguishable}
    D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right) = \int_{\cbar} \phibar^{\sran}(\cbar|\q) \log\left(\frac{\phibar^{\sran}(\cbar|\q)}{\phibar^{\s}(\cbar|\q)}\right) d\cbar>0.
\end{align}
 The distinguishable parameter set with $\q$ is $\Sobserve(\q) \deleq \left\{\S|D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right)>0\right\}$. 
\end{definition}


\begin{definition}[Global identification]\label{def:global_iden}
The true parameter $\sran$ is globally identifiable if for any $\q \in \Q$, $\Sobserve(\q)=\S \setminus \{\sran\}$. 
\end{definition}

\begin{definition}[Total variation distance]
For any belief $\theta \in \Delta(\S)$ and any strategy profile $\q \in \Q$, we define the total variation distance between $\mutheta\(\c|\q\)$ and $\phi^{\sran}(\c|\q)$ as follows: 
\begin{align*}
    \delta\(\mutheta(\cdot|\q), ~\phi^{\sran}(\cdot|\q)\)= \sup_{C \in \mathcal{B}}\left\vert\mutheta(C|\q)-\phi^{\sran}(C|\q)\right\vert.
\end{align*}
\end{definition}

\begin{theorem}\label{theorem:belief_convergence}
Given any sequence of strategy profiles $\(\qt\)_{\t =1}^{\infty}$, under assumptions (A1) and (A2), the sequence of beliefs $\(\thetat\)_{\t=1}^{\infty}$ generated by belief update in \eqref{eq:update_belief} converges to a belief vector $\thetabar \in \Delta(\S)$ with probability 1, and 
\begin{align}\label{eq:empirical_consistent}
    \lim_{\t \to \infty}  \delta\(\muthetat(\cdot|\qt),~ \phi^{\sran}(\cdot|\qt)\)=0, \quad w.p.1.
\end{align}
Moreover, if $\sran$ is globally identifiable, then $\thetabar=\thetasran$ with probability 1, where $\thetasran(\sran)=1$ is the complete information belief vector. 
\end{theorem}

\noindent\textbf{\emph{Proof of Theorem \ref{theorem:belief_convergence}.}}\\
\emph{Part 1:} We prove that $\thetat$ converges to a belief vector $\thetabar$ with probability 1. 

First, we show that for any $\s \in \S$, $\(\frac{\theta^\t(\s)}{\theta^\t(\sran)}\)_{\t=1}^{\infty}$ is a non-negative martingale, and hence converges to a belief vector $\thetabar$ with probability 1. Note that for any $\t=1, 2, \dots $, and any parameter $\s \in \S \setminus \{\sran\}$, we have the follows from \eqref{eq:update_belief}: 
\begin{align*}
\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}= \frac{\theta^{\t}(\s) \cdot \phibar^{\s}(\ct|\qt)}{\theta^{\t}(\sran) \cdot \phibar^{\sran}(\ct|\qt)}
\end{align*}
Now, consider any initial belief $\thetazero$, any sequence of aggregate strategies $\Qhis\deleq \(\q^j\)_{j=1}^{\t-1}$ and any sequence of realized outcomes $\Costhis\deleq \(\cj\)_{\j =1}^{\t-1}$ before stage $\t$, we can compute the expected value of $\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}$ conditioned on $\thetazero$, $\Qhis$ and $\Costhis$ as follows: 
\begin{align}\label{conditional_iterate}
\mathbb{E}\left[\left.\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}\right\vert \thetazero, \Qhis, \Costhis\right]&= \frac{\thetat(\s)}{\thetat(\sran)} \cdot \mathbb{E}\left[\left. \frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)}\right\vert \thetazero, \Qhis, \Costhis \right], 
\end{align}
where $\thetat$ is updated from $\thetazero$ based on $\Qhis$ and $\Costhis$ using \eqref{eq:update_belief}, and $\qt$ is derived from $\qt$ for all $\t$. 


We can check that the conditional expectation is 1: 
\begin{align*}
\mathbb{E}\left[\left. \frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)}\right\vert \thetazero, \Qhis, \Costhis \right]
=&\int_{\ct} \(\frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)} \) \cdot  \phibar^{\sran}(\ct|\qt) d \ct=1.
\end{align*}
Hence, for any $\t=1, 2, \dots$,  
\begin{align*}
\mathbb{E}\left[\left.\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}\right\vert \thetazero, \Qhis, \Costhis\right]= \frac{\thetat(\s)}{\thetat(\sran)}, \quad \forall \s \in \S.
\end{align*}
Additionally, from \eqref{eq:update_belief}, we know that $\frac{\theta^\t(\s)}{\theta^\t(\sran)} \geq 0$. Hence, the sequence $\(\frac{\theta^\t(\s)}{\theta^\t(\sran)}\)_{\t=0}^{\infty}$ is a non-negative martingale for any $\s \in \S$. From martingale convergence theorem, we conclude that $\frac{\theta^\t(\s)}{\theta^\t(\sran)}$ converges with probability 1. 

Next, we show that the sequence $\left(\log\thetat(\sran)\right)_{\t=1}^{\infty}$ is a submartingale, and converges with probability 1. We define $\mu (\ct|\theta^{\t}, \qt)\deleq\sum_{\s \in \S} \theta^{\t}(\s)\phibar^{\s}(\ct|\qt)$. From \eqref{eq:update_belief}, we have:
\begin{align*}
    &\mathbb{E}\left[\left.\log\theta^{\t+1}(\sran)\right\vert \thetazero, \Qhis, \Costhis\right]= \mathbb{E}\left[\left.\log\(\frac{\theta^{\t}(\sran)\phibar^{\sran}(\ct|\qt)}{\muthetat(\ct|\qt)}\)\right\vert \thetazero, \Qhis, \Costhis\right]\\
    =& \log\theta^{\t}(\sran) +\mathbb{E}\left[\left.\log\(\frac{\phibar^{\sran}(\ct|\qt)}{\muthetat(\ct|\qt)}\)\right\vert \thetazero, \Qhis, \Costhis\right]\\
    =&\log\theta^{\t}(\sran) +\int_{\ct} \phibar^{\sran}(\ct|\qt) \log\(\frac{\phibar^{\sran}(\ct|\qt)}{\muthetat(\ct|\qt)}\) d \ct \\
    =& \log\theta^{\t}(\sran)+  D_{KL}\(\phibar^{\sran}(\ct|\qt)||\muthetat(\ct|\qt)\) \geq \log\theta^{\t}(\sran),
\end{align*}
where the last inequality is due to the non-negativity of KL divergence between $\phibar^{\sran}(\ct|\qt)$ and $\muthetat(\ct|\qt)$. Therefore, the sequence $\left(\log\thetat(\sran)\right)_{\t=1}^{\infty}$ is a submartingale. Additionally, since $\log\thetat(\sran)$ is bounded above by zero, by the martingale convergence theorem, $\log\thetat(\sran)$ must converge with probability 1. Hence, $\thetat(\sran)$ must also converge with probability 1.

From the convergence of $\frac{\theta^\t(\s)}{\theta^\t(\sran)}$ and $\thetat(\sran)$, we can conclude that $\thetat(\s)=\frac{\theta^\t(\s)}{\theta^\t(\sran)} \cdot \thetat(\sran)$ converges with probability 1 for any $\s \in \S$. We denote the convergent vector as $\thetabar= \(\thetabar(\s)\)_{\s \in \S}$. We can check that for any $\t$, $\thetat(\s) \geq 0$ for all $\s \in \S$ and $\sum_{\s \in \S}\thetat(\s)=1$. Hence, $\thetabar$ must also satisfy $\thetabar(\s) \geq0$ for all $\s \in \S$ and $\sum_{\s \in \S}\thetabar(\s)=1$, i.e. $\thetabar$ is a feasible belief vector. 

\vspace{0.2cm}
\noindent\emph{Part 2:} We show that $\thetabar$ satisfies \eqref{eq:empirical_consistent} with probability 1. 

For any parameter $\s \in \S \setminus \{\sran\}$, we define $\Qhats$ as the set of strategy profiles, based on which the parameter $\s$ is distinguishable from $\sran$, i.e. 
\begin{align*}
   \Qhats \deleq \left\{\Q \left\vert D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right)>0\right.\right\}.
\end{align*}
The set $\Qhats \subseteq \Q$. For any $\q \in \Q \setminus \Qhats$, we must have $D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right)=0$. 

Since any sequence of strategy profiles $\(\qt\)_{\t=1}^{\infty}$ is a bounded sequence, from Bolzano-Weierstrass Theorem, we know that the sequence has at least one limit point. We define the set of all limit points of the sequence $\(\qt\)_{\t=1}^{\infty}$ as $\limpq \subseteq \Q$ and $\limpq$ is non-empty. We prove \eqref{eq:empirical_consistent} for the following three cases separately: 

\vspace{0.2cm}

\noindent\emph{(Case 1:)} For any $\s \in \S \setminus \{\sran\}$, the sequence of strategies $\(\qt\)_{\t=1}^{\infty}$ does not enter the set $\Qhats$ infinitely often for any $\s \in \S$. 

In this case, we can find a finite step $\T>0$ such that for any $\t >\T$, $\qt \notin \Qhats$ for all $\s \in \S$. Then, for any $\t > \T$ and any $\s \in \S$, since $\qt \notin \Qhats$, we have $D_{KL} \left(\phibar^{\sran}(\ct|\qt)||\phibar^{\s}(\ct|\qt)\right)=0$, which implies $\phi^\s(\ct|\qt)=\phi^{\sran}(\ct|\qt)$ for all $\ct$. Then, for any $\thetat$, we have $\muthetat\(\ct| \qt\)= \sum_{\s \in \S} \thetat(\s)\phi^\s(\ct|\qt)=\phi^{\sran}(\ct|\qt)$ for all $\ct$. Hence, $D_{KL} \left(\phibar^{\sran}(\ct|\qt)||\muthetat\(\ct| \qt\)\right)=0$. Therefore, we can conclude that $\thetabar$ must satisfy \eqref{eq:empirical_consistent}.  

\noindent\emph{(Case 2:)} For any $\s \in \S$, we have $\limpq \cap \Qhats = \emptyset$.

To begin with, we argue that for any $\epsilon>0$, there exits a finite $\T>0$ such that for any $\t >\T$, $d\(\qt, \limpq\)<\epsilon$. Assume for the contrary that such finite $\T$ cannot be found, then there must exist a sub-sequence of strategy profiles $\(\qtk\)_{\k=1}^{\infty}$ such that $d\(\qtk, \limpq\)>\epsilon$ for all $\tk$. Since the infinite number of strategy profiles in the sub-sequence belong to the bounded closed set $\Q$, again from Bolzano-Weierstrass Theorem, we know that the sub-sequence must have at least one limit point, denoted as $\hat{\q}'$. Since $d\(\qtk, \limpq\)>\epsilon$ for all $\tk$, $\hat{\q}' \geq \epsilon>\frac{\epsilon}{2}$, and hence $\hat{\q}' \notin \Q'$. We then obtain a contradiction since $\Q'$ is the set of all limit points. 

In this case, for any $\q' \in \limpq$, $D_{KL} \left(\phibar^{\sran}(\cbar|\q')||\phi^\s\(\c| \q'\)\right)=0$. From assumption (A1), we know that for any $\epsilon>0$, we can find a positive number $\delta >0$ such that if $|\q-\q'|<\delta$, then  $\delta\(\phi^\s(\cdot|\qt),~ \phi^{\sran}(\cdot|\qt)\)<\epsilon$. Based on the above-mentioned argument, we know that there exists a finite step number $\T>0$ such that for all $\t>\T$, $ d\(\qt, \limpq\)<\delta$, i.e. for any $\t > \T$, $\exists \q' \in \limpq$ such that $|\qt-\q'|<\delta$. We can thus prove \eqref{eq:empirical_consistent} by concluding that for any $\epsilon>0$, there exists a $\T>0$ such that for any $\t>\T$,  $\delta\(\phi^\s(\cdot|\qt),~ \phi^{\sran}(\cdot|\qt)\)<\epsilon$. 



\noindent\emph{(Case 3:)} There exists a parameter $\s \in \S$ such that the sequence $\(\qt\)_{\t=1}^{\infty}$ enters the set $\Qhats$ infinitely often, and the joint set $\limpq \cap \Qhats \neq \emptyset$. We denote the set of such parameters as $\Sdagger$.


Our goal is to show that for any $\s \in \Sdagger$, $\thetabar(\s)=0$ with probability 1. By iteratively applying the belief update in \eqref{eq:update_belief}, we can write the belief $\thetat$ as follows: 
\begin{align}\label{eq:sequence_update}
    \thetat(\s)= \frac{\theta^1(\s) \prod_{\j=1}^{\t-1}\phibar^{s}(\cj|\q^j)}{\sum_{\s' \in \S} \theta^1(\s') \prod_{\j=1}^{\t-1}\phibar^{s'}(\cj|\q^j)}, \quad \forall \s \in \S.
\end{align}
We define $\Phi^\s(\Costhis|\Qhis)$ as the density function of the history of the realized outcomes $\Costhis$ conditioned on the history of aggregate strategies $\Qhis$ before stage $\t$, i.e. $\Phi^\s(\Costhis|\Qhis) \deleq \prod_{\j=1}^{\t-1}\phibar^{s}(\cj|\q^j)$. Then, we simplify \eqref{eq:sequence_update} as follows: 
\begin{align}
    \thetat(\s)&= \frac{\theta^1(\s) \Phi^\s(\Costhis|\Qhis)}{\sum_{\s' \in \S} \theta^1(\s') \Phi^{\s'}(\Costhis|\Qhis)} \leq \frac{\theta^1(\s) \Phi^\s(\Costhis|\Qhis)}{ \theta^1(\s) \Phi^{\s}(\Costhis|\Qhis)+ \theta^1(\sran) \Phi^{\sran}(\Costhis|\Qhis)}\notag\\
    &=\frac{\theta^1(\s) \frac{\Phi^\s(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}}{ \theta^1(\s) \frac{\Phi^{\s}(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}+ \theta^1(\sran)}\label{eq:bound_theta}
\end{align}
Hence, if we can prove that the likelihood ratio $ \frac{\Phi^\s(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}$ converges to 0 as $\t$ goes to infinity for all $\s \in \Sdagger$, then $\theta(\s)$ must also converge to 0. %To begin with, we compute the log-likelihood ratio as follows:  



Since the sequence $\(\qt\)_{\t=1}^{\infty}$ enters the set $\Qhats$ infinitely often, we have a sub-sequence of strategy profiles in the set $\Qhats$ as $\(\qtk\)_{\k=1}^{\infty}$. For any $\t \in  \{1, 2, \dots\} \setminus \{\t_1, \t_2, \dots\}$, since $\qt \notin \Qhats$, the KL-divergence $D_{KL}\(\phibar^{\sran}(\cj|\loadj)||\phibar^{\s}(\cj|\loadj)\)=0$, which implies that $\phibar^{\s}(\cj|\loadj)=\phibar^{\sran}(\cj|\loadj)$ with probability 1. Then, we can write the likelihood ratio as follows:
\begin{align}\label{eq:likelihood}
    \lim_{\t \to +\infty}\frac{\Phi^\s(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}=  \sum_{\t=1}^{+\infty} \frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)}=  \sum_{\k=1}^{+\infty} \frac{\phibar^{\s}(\ctk|\qtk)}{\phibar^{\sran}(\ctk|\qtk)}.
\end{align}


We further break the sequence $\(\qtk\)_{\k=1}^{\infty}$ into converging sub-sequences: Since $\(\qtk\)_{\k=1}^{\infty}$ is a bounded infinite sequence, we must be able to find a converging sub-sequence, denoted as $\hat{\Q}^1 \deleq \(\q^{\tk^1}\)_{\k=1}^{\infty}$, and the limit point is $\qhat^1$. If the remaining strategy profiles are finite, then we denote the remaining strategy profiles as $\hat{\Q}^0$. Otherwise, we can find the second converging sub-sequence, denoted as $\hat{\Q}^2 \deleq \(\q^{\tk^2}\)_{\k=1}^{\infty}$, and the limit point is $\qhat^2$. This process is continued iteratively

then we have a single converging (sub)-sequence ($m=1$), and we denote the limit point as $\qhat^1$. If $\(\qtk\)_{\k=1}^{\infty}$ is a divergent sequence, then can find a converging sub-sequence, denoted as 


We will show that $\thetabar(\s)=0$ for any such $\s$ with probability 1. 

From the definition of limit point, for any strategy profile $\qbar \in \limpq \cap \Qhats$, we can find a sub-sequence $\(\qtk\)_{\k =1}^{\infty}$ such that $\lim_{\k \to \infty} \qtk=\qbar$, and $D_{KL} \left(\phibar^{\sran}(\cbar|\qbar)||\phibar^{\s}(\cbar|\qbar)\right)>0$. We next show that 






Then from the definition of limit point, we know that for any $\q \in \limpq$, there exists a sub-sequence 
\QEDA

==> complete.tex <==
%\[=======\text{\textcolor{blue}{New text starts from here}}=======\]
\section{Convergence to Complete Information Equilibrium}\label{sec:discussion}
We present a sufficient and necessary condition under which all fixed points are complete information fixed points. We also derive a set of sufficient conditions on fixed points and the average payoff functions of the game, which ensure that the strategy played in the fixed point is equivalent to a complete information equilibrium although the fixed point belief may not have complete information of the true parameter. Finally, we discuss how players can learn the true parameter and find the complete information equilibrium when such conditions are not satisfied. 


Recall from \eqref{eq:FP}, if all fixed points in $\FP$ are complete information fixed points, then any $\theta \in \Delta(\S)$ other than the complete information belief $\thetasran$ cannot be a fixed point belief. Therefore, from Theorem \ref{theorem:convergence_eq}, all fixed points being complete information fixed points is equivalent to the condition that the support set of any $\theta \in \Delta(\S)\setminus \{\thetasran\}$ contains at least one parameter that is not payoff-equivalent to the true parameter $\sran$ for any equilibrium strategy profile corresponding to $\theta$. %there does not exist any $\theta \in \Delta(\S) \setminus \{\sran\}$ such that parameters in $[\theta]$ are all payoff-equivalent to $\sran$ given any $\q \in \EQ(\theta)$. 
\begin{corollary}\label{cor:complete_belief}
    The fixed point set $\FP \equiv \{\(\thetasran, \qsran\)|\qsran \in \EQ(\thetasran)\}$ if and only if $[\theta] \setminus \Sequiv\(\q\)$ is non-empty for any $\theta \in \Delta(\S) \setminus \{\thetasran\}$ and any $\q \in \EQ(\theta)$. 
\end{corollary}

From Proposition \ref{prop:complete}, we obtain that the condition in Corollary \ref{cor:complete_belief} is also the sufficient and necessary condition of the existence of globally stable fixed points. Therefore, under this condition, the learning dynamics recovers the complete information environment with probability 1. 

On the other hand, when the condition in Corollary \ref{cor:complete_belief} is not satisfied, there must exist at least one fixed point $\(\thetabar, \qbar\) \in \FP$ such that $\thetabar \neq \thetasran$. In this case, the true parameter $\sran$ is not fully identified by $\thetabar$, and $\qbar$ may or may not be a complete information equilibrium. Next, we present a condition under which the fixed point strategy is a complete information equilibrium even when $\thetabar \neq \thetasran$:
\begin{proposition}\label{prop:complete}
Given fixed point belief $\thetabar$, $\EQ(\thetabar)=\EQ(\thetasran)$ if the payoff function $\usi(\qi, \qmi)$ is concave in $\qi$ for all $\i \in \I$ and all $\s \in [\thetabar]$ and there exists a positive number $\loaddelta >0$ such that $[\thetabar] \subseteq \Sequiv(\q)$ for any $\q \in N_{\delta}\(\EQ(\thetabar)\)$. 
\end{proposition}

We can verify the condition that $\exists \loaddelta >0$ such that $[\thetabar] \subseteq \Sequiv(\q)$ for all $\q \in N_{\delta}\(\EQ(\thetabar)\)$ by analyzing whether or not the KL-divergence $D_{KL}\(\phi^s(\c|\q)||\phi^{\s'}(\c|\q)\)$ between each pair of parameters $\s, \s' \in [\thetabar]$ remains zero under perturbations of $\q \in \EQ(\thetabar)$. 

Proposition \ref{prop:complete} is intuitive: For any fixed point belief $\thetabar$ and any fixed point strategy $\qbar \in \EQ(\thetabar)$, since $\qbar_i$ is a best response strategy of $\qbar_{\mi}$, $\qbar_i$ is a local maximizer of the expected payoff function $\mathbb{E}_{\thetabar}[u_i^s(\qi, \qbar_{\mi})]$. From the condition in Proposition \ref{prop:complete}, we know that the value of the expected payoff function is identical to that with the true parameter $\sran$ for $\qi$ in a small neighborhood of $\qbar_i$. Therefore, $\qbar_i$ must also be a local maximizer of the payoff function with the true parameter $u_i^{\sran}(\qi, \qbar_{\mi})$. Since the payoffs are concave functions of the strategies for any $\s \in [\thetabar]$, $\qbar_i$ is a global maximizer of $u_i^{\sran}(\qi, \qbar_{\mi})$. Thus, any $\qbar \in \EQ(\thetabar)$ is an equilibrium of the game with complete information of $\sran$. We include the formal proof in Appendix \ref{apx:proof}. 



We introduce a modified coordination game that satisfies the condition in Proposition \ref{prop:complete}. 

\begin{example}[Coordination with increasing penalty]\label{ex:concave}
{\normalfont We consider a modified version of the coordination game in Example \ref{ex:coordinate}, in which player 1 chooses strategy $\q_1 \in [0, 2]$ and player 2 chooses strategy $\q_2 \in [1,4]$. Players pay a cost that increases with the difference between their strategies $|\q_1- \q_2|$. In particular, when $|\q_1- \q_2|<1$, the cost is $\(\q_1- \q_2\)^2$. If $|\q_1- \q_2|>1$, then the cost is $\(1+\s\(|\q_1-\q_2|-1\)\)^2$, where each unit of strategy difference that exceeds 1 is penalized by $\s$. The unknown parameter $\s$ is in the set $\S = \{\s_1=2, \s_2 =4\}$, and the true parameter is $\sran=\s_1$. Similar to Example \ref{ex:coordinate}, player 1 prefers to choose small $\q_1$, and player 2 prefers high $q_2$. The payoff of each player is given as follows: 
\begin{align*}
    \c_1 &= \left\{
    \begin{array}{ll}
    -\(\q_1- \q_2\)^2- q_1 +\epsilon_1, & \quad \text{If $|\q_1-\q_2|\leq 1$} \\
    -\(1+\s\(|\q_1-\q_2|-1\)\)^2- q_1 +\epsilon_1, & \quad \text{If $|\q_1-\q_2|> 1$}
    \end{array}
    \right.\\
    \c_2 &= \left\{
    \begin{array}{ll}
    -\(\q_1- \q_2\)^2+q_2 +\epsilon_1, & \quad \text{If $|\q_1-\q_2|\leq 1$} \\
    -\(1+\s\(|\q_1-\q_2|-1\)\)^2+q_2 +\epsilon_1, & \quad \text{If $|\q_1-\q_2|> 1$,}
    \end{array}
    \right.
\end{align*}
where $\epsilon_1$ and $\epsilon_2$ are the noise terms with zero means. 

For any belief $\theta \in \Delta(\S)$, the set of equilibrium strategy $\EQ(\theta)$ is given by: 
\begin{align*}
\EQ(\theta)=\{\(\q_1, \q_2\) \in \Q\left\vert \(\q_2-\q_1\)=1/2\right.\}.
\end{align*}
We can check that the conditions in Proposition \ref{prop:complete} are satisfied in this example. Therefore, even though players do not have complete information of the unknown parameter, any fixed point strategy is a complete information equilibrium.}
\end{example}



If $\thetabar \neq \thetasran$ and the conditions in Proposition \ref{prop:complete} are not satisfied, then the fixed point strategy $\qbar$ may not be a complete information equilibrium. In general, players' payoffs $u^{\sran}_i(\qbar)$ given $\qbar$ may be higher or lower than $u^{\sran}_i(\qsran)$ with a complete information equilibrium $\qsran$. Recall from Example \ref{ex:potential}, the fixed point strategy profile $\qbar=\(0.5, 0.5\)$ has higher payoff for both players than the complete information strategy profile $\qsran=\(2/3, 2/3\)$. However, in many other games, players may want to learn the complete information equilibrium either because the payoffs under the complete information equilibrium are higher than the payoffs given by other fixed point strategies\footnote{In \cite{wu2019learning}, we proved that in routing games on series-parallel networks, average equilibrium costs of players are higher when they have less than perfect information of the network condition.}, or simply because they prefer to identify the true parameter.  

We now outline a procedure that players can use to distinguish the true parameter $\sran$ from other parameters in the set $[\thetabar]$ and learn the complete information equilibrium after the states of the learning dynamics have converged to a fixed point $\(\thetabar, \qbar\)$. Note that any two parameters $\s, \s' \in [\thetabar]$ must be payoff equivalent given the fixed point strategy $\qbar$. Therefore, to distinguish $\s$ from $\s'$ based on the realized payoffs, players need to take strategy profiles for which $\s$ and $\s'$ are not payoff equivalent. One simple example is when the average payoff functions are affine in $\q$, i.e. $\c_i=\alpha^s_i \q+\beta_i^s+\epsilon_i^s$ for all $\i \in \I$, where the vectors $\alpha^\s = \(\alpha^\s_\i\)_{\i\in I}$ and $\beta^\s= \(\beta_i^\s\)_{\i \in \I}$ depend on the unknown parameter $\s$. In this case, players can distinguish all $\s \in [\thetabar] \setminus \{\sran\}$ from the true parameter $\sran$ by repeatedly taking any strategy that is in a local neighborhood of $\qbar$. This is because two affine payoff functions can only have identical values for at most on one strategy profile. Hence $\qbar$ must be the only strategy for which $\s \in [\thetabar] \setminus \{\sran\}$ is payoff equivalent to $\sran$. Moreover, since players' payoff functions are continuous in their strategies, local perturbation of $\qbar$ only changes the players' average payoffs by a small number. 


On the other hand, when the payoffs are nonlinear functions, parameters in $[\thetabar]$ may remain to be payoff equivalent in the local neighborhood of $\qbar$, but result in different payoffs for strategies outside of the neighborhood. Then, local perturbations of $\qbar$ may not identify the true parameter, and players need to repeatedly play strategies in set $\widehat{\Q}^\s \deleq \{\q \in \Q| \s \not \in \Sequiv(\q)\}$ in order to distinguish each $\s \in [\thetabar]$ with the true parameter $\sran$. However, some players' payoffs given $\q \in \widehat{\Q}^\s$ may be significantly lower than their payoffs at the fixed point. Therefore, players need to be incentivized to take such strategies in order to learn the true parameter. The design of such mechanism is beyond the scope of this article. 





==> correspondence.tex <==
%%novalidate
\section{Equilibria Sets and Best-response correspondences}\label{sec:set_valued}
In this section, we show that our convergence and stability results in Secs. \ref{sec:equilibrium} and \ref{sec:br} can be extended to situations where the equilibrium function $\gwe(\theta)$ and the best-response function $\gbr(\theta, \q)$ are set-valued. We present the results for set-valued equilibrium function in Sec. \ref{subsec:eq_set}, and set-valued best-response function in Sec. \ref{subsec:br_set}. We also briefly discuss the extension of learning with smoothed best-response strategy update. 

When the game has multiple equilibria and the stepsizes $\ait$ can take any number in $[0,1]$, the sequence of beliefs $\(\thetat\)_{\t =1}^{\infty}$ still converge to a fixed point belief $\thetabar$, but the sequence of strategies $\(\qt\)_{\t=1}^{\infty}$ may not converge. We define the limit point set $\limitq$ as the set of strategies, which are the limit points of the subsequences of strategies. 
\begin{definition}[Limit strategy set]\label{def:limit_point}
The set $\limitq \subseteq \Q$ is the limit set of the sequence $\(\qt\)_{\t=1}^{\infty}$ if for any $\qbar \in \limitq$, we can find a converging subsequence of strategy profiles $\(\qtk\)_{\k=1}^{\infty}$ such that that $\lim_{\k \to \infty} \qtk=\qbar$. 
\end{definition}
Then, we extend Definition \ref{def:payoff_equivalence} to define the set of payoff equivalent parameters given the limit point set $\limitq$ as $\Sequiv(\limitq) \deleq \cap_{\qbar \in \limitq} \Sequiv(\qbar)$. 




The next proposition shows that the strategies converge to the set of equilibrium strategy profile $\gwe(\thetabar)$. Moreover, the convergent belief $\thetabar$ only assigns positive probability on parameters that are payoff equivalent to $\sran$ based on the limit set $\Qbar$. 

\begin{proposition}\label{prop:convergence_set}
For any initial state~$(\theta^1, \q^1)$, the sequence of beliefs $(\thetat, \qt)_{\t=1}^{\infty}$ satisfies: 
\begin{subequations}\label{eq:set_eq_convergence}
\begin{align}
    \lim_{\t \to \infty} \thetat &=\thetabar, \quad w.p.1, \\
    \lim_{\t \to \infty} d\(\qt, \gwe(\thetabar)\)&=0, \quad w.p.1,
\end{align}
\end{subequations}
where $d\(\qt, \gwe(\thetabar)\) \deleq \inf_{\q \in \gwe(\thetabar)} \|\qt-\q\|$ is the distance between $\qt$ and the equilibrium set $\gwe(\thetabar)$. Moreover, the limit set of the strategy sequence $\(\qt\)_{\t=1}^{\infty}$ is $\limitq \subseteq \gwe(\thetabar)$. The belief $\thetabar$ satisfies $[\thetabar] \subseteq \Sequiv(\limitq)$ with probability 1. \end{proposition}

That is, populations eventually strategies in the equilibrium set of the game with belief $\thetabar$. A parameter $\s$ is excluded from the belief $\thetabar$ if a strategy subsequence converges to an equilibrium strategy $\qbar \in \gwe(\thetabar)$, and $\s$ and $\sran$ are not payoff equivalent given $\qbar$. The idea of the proof is to first find the converging subsequence. Then, from Part 3 in the proof of Theorem \ref{theorem:convergence}, we can show that the likelihood ratio $\frac{\thetat(\s)}{\thetat(\sran)}$ updated given the subsequence of strategies either converges to zero exponentially fast (when $\phibar^{\s}(\c|\qbar)$ is absolutely continuous with $\phibar^{\sran}(\c|\qbar)$) or becomes zero in finite steps (when $\phibar^{\s}(\c|\qbar)$ is not absolutely continuous with $\phibar^{\sran}(\c|\qbar)$). 


Moreover, since the strategy $\qt$ converges to the set of equilibrium $\gwe(\thetabar)$ instead of a particular fixed point strategy, our definition of local stability as in Definition \ref{def:local} needs to be slightly changed to incorporate the set-valued equilibrium function. In particular, we say that $\(\thetabar, \gwe(\thetabar)\)$ is locally stable if for any $\thetaepfin, \loadepfin>0$ and any probability $\gamma<1$, we can find $\thetaep, \loadep$ such that if $\thetazero \in \neighinitheta \deleq \{\theta|\|\theta-\thetabar\|<\thetaep\}$ and $\q^1 \in \neighiniload \deleq \{\q| d\(\q, \gwe(\thetabar)\)<\loadep\}$, then $\pro(\(\thetat, \qt\) \in \neighinftheta \times \neighinfload)>\gamma$, where $\neighinftheta \deleq \{\theta|\|\theta-\thetabar\|<\thetaepfin\}$ and $\neighinfload \deleq \{\q| d\(\q, \gwe(\thetabar)\)<\loadepfin\}$. Analogously, we say that $\(\thetabar, \gwe(\thetabar)\)$ is globally stable if for any initial state $\(\theta^1, \q^1\)$, the state of the learning dynamics converge to $\(\thetabar, \gwe(\thetabar)\)$ with probability 1. 



==> methodology.tex <==
%%novalidate

We prove Theorem \ref{theorem:convergence_eq} in three lemmas. Firstly, Lemma \ref{lemma:theta_eq} establishes the convergence of beliefs $\(\thetat\)_{\t=1}^{\infty}$ by showing that both sequences $\left(\frac{\thetat(\s)}{\thetat(\sran)}\right)_{\t=1}^\infty$ and $\left(\thetat(\sran)\right)_{\t=1}^{\infty}$ are non-negative martingales, and hence converge.  

\begin{lemma}\label{lemma:theta_eq}
$\lim_{\t \to \infty} \thetat=\thetabar$, where $\thetabar = \gwe(\thetabar) \in\Delta(S)$.
\end{lemma}








Secondly, Lemma \ref{lemma:q_eq} shows that the sequence of strategies $\(\qit\)_{\t=1}^{\infty}$ converges to an equilibrium strategy of game $\G$ for belief $\thetabar$ as in \eqref{subeq:eq_fixed}. 
\begin{lemma}\label{lemma:q_eq}
$\lim_{\t \to \infty} \qt = \qbar$, where $\qbar \in \EQ(\thetabar)$.
\end{lemma}
By using iterative updates \eqref{eq:eq_update}, we can write $\qt$ as a linear combination of the initial strategy profile $\q^1$ and equilibrium sequence $\(\gwe(\theta^j)\)_{j=2}^{\t}$. The convergence of strategies follow from the convergence of $\(\thetat\)_{\t=1}^{\infty}$ in Lemma \ref{lemma:theta_eq} and Assumptions \textbf{(A1)}--\textbf{(A2)}.  




Thirdly, using the convergence of both $\(\thetat\)_{\t=1}^{\infty}$ and $\(\qit\)_{\t=1}^{\infty}$, Lemma \ref{lemma:consistency} shows that the belief of any $\s$ that is not payoff-equivalent to $\sran$ given $\qbar$ must converge to $0$, i.e. $\thetabar$ satisfies \eqref{eq:exclude_distinguished}. This concludes proof of Theorem \ref{theorem:convergence_eq}. Besides, Lemma \ref{lemma:consistency} also provides a convergence rate of beliefs. 
\begin{lemma}\label{lemma:consistency}
Any fix point $\(\thetabar, \qbar\)$ of learning dynamics satisfies \eqref{eq:exclude_distinguished}. Furthermore, for any $\s \in \S\setminus \Sequiv(\qbar)$, if $\phibar^{\sran}(\chat|\qbar) \ll \phibar^{\s}(\chat|\qbar)$, then $\thetat(\s)$ converges to 0 exponentially fast: 
\begin{align}
    \lim_{\t \to \infty} \frac{1}{\t} \log(\thetat(\s))=-D_{KL}(\phibar^{\sran}(\cbar|\qbar)||\phibar^{\s}(\cbar|\qbar)). \quad  w.p.~1\label{eq:rate}
\end{align}
Otherwise, there exists a finite positive integer $\Tstar$ such that $\thetat(\s)=0$ for all $\t>\Tstar$ w.p. 1. 
\end{lemma}


\begin{lemma}[\cite{perkins2013asynchronous}]\label{lemma:asynchronous}
Under assumptions \textbf{(A3)} -- \textbf{(A6)}, if $\xi^{\t}=\(\xi_i^\t\)_{\i \in \I}$ is bounded for all $\t$ and $\lim_{\t \to \infty} \xi^{\t}=0$, then the sequence $\(\qt\)_{\t=1}^{\infty}$ given by \eqref{eq:rewrite_dynamics} converges to the equilibrium set $\EQ(\thetabar)$ for any $\thetabar \in \Delta(\S)$. 
\end{lemma}

Based on \textbf{(A5)}, we can show that for any sequence of beliefs $\(\thetat\)_{\t=1}^{\infty}$ that converge to $\thetabar$, the sequence $\(\xi^{\t}\)$ indeed converges to zero. 
\begin{lemma}\label{lemma:residual_zero}
Under Assumption \textbf{(A5)}, for any belief sequence $\(\thetat\)_{\t=1}^{\infty}$ such that $\lim_{\t \to \infty} \thetat = \thetabar$, $\xi^{\t}=\(\xi_i^\t\)_{\i \in \I}$ is bounded for all $\t$ and $\lim_{\t \to \infty} \xi^{\t}=0$. 
\end{lemma}

The proof of Lemma \ref{lemma:residual_zero} is included in Appendix \ref{apx:proof}. From Lemmas \ref{lemma:asynchronous} and \ref{lemma:residual_zero}, we can conclude that as the beliefs $\(\thetat\)_{\t=1}^{\infty}$ converge to a fixed point belief vector $\thetabar$, the strategies $\(\qt\)_{\t =1}^{\infty}$ also converge to the equilibrium set $\EQ(\thetabar)$ corresponding to fixed point belief $\thetabar$. 
\begin{lemma}\label{lemma:q_br}
Under Assumptions \textbf{(A3)} -- \textbf{(A6)}, $\lim_{\t \to \infty} d \(\qt, \EQ(\thetabar)\)=0$ with probability 1. 
\end{lemma}



Now, recall from Lemma \ref{lemma:consistency} in Sec. \ref{subsec:convergence_eq} that in learning with equilibrium strategies, any fixed point belief $\thetabar$ identifies the true parameter $\sran$ in the payoff-equivalent parameter set given the corresponding fixed point strategy $\qbar$. In learning with best response strategies, if the game with fixed point belief $\thetabar$ has multiple equilibria, then the strategy profiles $\(\qt\)_{\t=1}^{\infty}$ converge to the equilibrium set $\EQ(\thetabar)$, but not necessarily converge to a single fixed point strategy. Thus, we need the notion of the limit set of $\(\qt\)_{\t=1}^{\infty}$:
\begin{definition}[Limit set]\label{def:limit_point}
Set $\limitq \subseteq \Q$ is the limit set of the sequence $\(\qt\)_{\t=1}^{\infty}$ if for any $\qbar \in \limitq$, there exists a subsequence of strategy profiles $\(\qtk\)_{j=1}^{\infty}$ such that $\lim_{j \to \infty} \qtk=\qbar$. 
\end{definition}
That is, limit set $\Qbar$ is the set of strategies that are limit points of converging subsequences in $\(\qt\)_{\t=1}^{\infty}$. The limit set must be nonempty since the feasible strategy set $\Q$ is bounded. From Lemma \ref{lemma:q_br}, we know that $\limitq \subseteq \EQ(\thetabar)$.  

Analogous to Definition \ref{def:payoff_equivalence}, we define payoff-equivalent parameters on a set of strategies:
\begin{definition}\label{def:set_payoff}
The set of parameters that are payoff-equivalent to $\sran$ on a set $\widehat{\Q} \subseteq \Q$ is:
\begin{align*}
  \Sequiv(\widehat{Q})\deleq \left\{\S|D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right)=0,  ~ \forall \q \in \widehat{\Q}\right\}. 
\end{align*}
\end{definition}


We now show that in learning with best response strategies, $\thetabar$ only assigns positive probability on parameters that are payoff-equivalent to $\sran$ on the set $\limitq$. That is, the fixed point belief $\thetabar$ consistently estimates the payoff distribution of the strategies in the limit set $\limitq$. 
\begin{lemma}\label{lemma:consistency_br}
$[\thetabar] \subseteq \Sequiv(\limitq)$ with probability 1, where $\limitq \subseteq \EQ(\thetabar)$ is the limit set of the strategy sequence $\(\qt\)_{\t=1}^{\infty}$. 
\end{lemma}
The proof of Lemma \ref{lemma:consistency_br} is as follows: For any $\qbar \in \limitq$, from Definition \ref{def:limit_point}, there must exist a subsequence of strategies in $\(\qt\)_{\t=1}^{\infty}$ that converges to $\qbar$. Then, we use the same approach developed in Lemma \ref{lemma:consistency} to show that the belief ratio $\(\frac{\thetat(\s)}{\thetat(\sran)}\)_{\t=1}^{\infty}$ converges to 0 for any $\s \in \S \setminus \Sequiv(\qbar)$. Since this argument holds for any $\qbar \in \Qbar$, we know that $\thetabar(\s)$ is positive only if $\s$ is payoff-equivalent to $\sran$ for all $\qbar \in \Qbar$. The proof of this lemma is in Appendix \ref{apx:proof}. 


Based on Lemmas \ref{lemma:theta_eq}, \ref{lemma:q_br} and \ref{lemma:consistency_br}, we obtain the following convergence result: 




==> proof_applications.tex <==
%%novalidate
% !TEX root = main041620.tex
\noindent\textbf{\emph{Proof of Proposition \ref{prop:complete}.}} 

\vspace{0.2cm}
\noindent\textbf{\emph{Proof of Proposition \ref{prop:map_convergence}}
.} 
First, since the Bayesian belief $\thetat$ given by \eqref{eq:update_belief} converges to a fixed point belief $\thetabar$ and $\thetat_M = \argmax_{\s \in \S} \thetat(\s)$, we know that $\lim_{\t \to \infty} \thetat_M= \thetabar_M$, where $\thetabar_M = \argmax_{\s \in \S} \thetabar(\s)$ with probability 1. Second, analogous to Lemma \ref{lemma:q_eq}, we can show that $\lim_{\t \to \infty} \qt= \qbar=\gwe(\thetabar_M)$ in learning with equilibrium strategies under \textbf{(A1)} -- \textbf{(A2)}. Additionally, we know from Lemma \ref{lemma:consistency} that $\lim_{\t \to \infty}\thetat(\s) = 0$ for $\s \in \S \setminus \Sequiv(\qbar)$. Therefore, $\thetabar_M = \argmax_{\s \in \S} \thetabar(\s)$ must be in the set $\Sequiv(\qbar)$. Finally, analogous to Lemma \ref{lemma:q_br}, we can show that $\lim_{\t \to \infty} d\(\qt, \EQ(\thetabar_M)\)=0$ in learning with best response strategies under \textbf{(A3)} -- \textbf{(A6)}. Additionally, we know from the proof of Lemma \ref{lemma:constrained_set} that $\lim_{\t \to \infty}\thetat(\s) = 0$ for $\s \in \S \setminus \Sequiv(\Qbar)$, where $\Qbar$ is the limit set of sequence $\(\qt\)_{\t=1}^{\infty}$. Therefore, $\thetabar_M = \argmax_{\s \in \S} \thetabar(\s)$ must be in the set $\Sequiv(\Qbar)$. 
\QEDA





==> proof_games.tex <==
%%novalidate

\noindent\textbf{\emph{Proof of Proposition \ref{prop:potential}.}}
We prove \emph{1-3} in sequence: 

1. We can show that the function $\mathbb{E}_{\theta}[\Psi^s(\q)]$ is a potential function of game $G_P$ with belief $\theta$: 
\begin{align*}
&\mathbb{E}_{\theta}[\Psi^s(\qi, \qmi)] - \mathbb{E}_{\theta}[\Psi^s(\qi', \qmi)]= \sum_{\s \in \S} \theta(\s)\(\usi(\qi, \qmi) - \usi(\qi', \qmi)\)\\
&= \mathbb{E}_{\theta}[\usi(\qi, \qmi)] - \mathbb{E}_{\theta}[\usi(\qi', \qmi)], \quad \forall \i \in \I, \quad \forall \qi, \qi' \in \Qi, \quad \forall \qmi \in \Qmi.
\end{align*}
Therefore, the equilibrium set can be solved as $\EQ(\theta)=\argmax_{\q \in \Q} \mathbb{E}_{\theta}[\Psi^s(\q)]$. Note that $\mathbb{E}_{\theta}[\Psi^s(\q)]$ is a continuous function in $\q$ and $\theta$, and the set $\Q$ is a closed convex set. From Berge's maximum theorem, we obtain that the equilibrium set is upper-hemicontinuous in $\theta$. If the function $\Psi^s(\q)$ is strictly concave in $\q$ for all $\s \in \S$, then $\mathbb{E}_{\theta}[\Psi^s(\q)]$ is also strictly concave in $\q$. Therefore, the optimal solution set $\argmax_{\q \in \Q} \mathbb{E}_{\theta}[\Psi^s(\q)]$ is a singleton set, and the unique equilibrium strategy profile $\gwe(\theta)$ must be continuous in $\theta$. 


2. For any player $\i \in \I$ and any other players' strategy $\qmi \in \Qmi$, the set of best response strategies is solved as $\BR_i(\theta, \qmi)=\argmax_{\qi \in \Qi} \mathbb{E}_{\theta}[\Psi^s(\qi, \qmi)]$. Again from the Berge's maximum theorem, since the potential function $\mathbb{E}_{\theta}[\Psi^s(\qi, \qmi)]$ is continuous in $\theta$, $\qi$ and $\qmi$, we know that $\BR_i(\theta, \qmi)$ must be upper-hemicontinuous in $\theta$ and $\qmi$. Since the function $\mathbb{E}_{\theta}[\Psi^s(\q)]$ is concave in $\qi$ and $\Qi$ is a convex bounded set, we know that the set of optimal solutions $\BR_i(\theta, \qmi)$ must also be a convex set. 


3. For any $\theta$ and any solution $\tilde{\q}(\tau)$ of the differential inclusion \eqref{eq:differential_inclusion}, we consider the expected value of the potential function $\mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))]$. Since $\Psi^s(\tilde{q}(\tau))$ is differentiable in $\tilde{q}$, we can compute the derivative of $\mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))]$ with respect to $\tau$:
\begin{align*}
&\frac{d \mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))]}{d \tau} = \sum_{\s \in \S} \theta(\s) \sum_{\i \in \I} \nabla_{\qdiff_i(\tau)}\mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))] \cdot \frac{d \qdiff_i(\tau)}{d \tau}\\
\stackrel{\eqref{eq:differential_inclusion}}{\in}&\sum_{\s \in \S} \theta(\s) \( \sum_{\i \in \I} \nabla_{\qdiff_i(\tau)}\mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))] \cdot  \alpha_i \(\BRi(\theta, \qdiff_{\mi}(\tau))- \qdiff_i(\tau)\)\),
\end{align*}
where $\alpha_i \in [\nu, 1]$ and $\epsilon>0$. 
Since $\mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))]$ is concave in $\qdiff_i(\tau)$, for any best response strategy $\gibr(\theta, \qdiff_{\mi}(\tau)) \in \BRi(\theta, \qdiff_{\mi}(\tau))$, we have: 
\begin{align*}
\nabla_{\qdiff_i(\tau)}\mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))] \(\gibr(\theta, \qdiff_{\mi}(\tau))- \qdiff_i(\tau)\)\geq \mathbb{E}_{\theta}[\Potentials\(\gibr(\theta, \qdiff_{\mi}(\tau)), \qdiff_{\mi}(\tau)\)] - \mathbb{E}_{\theta}[\Potentials(\qdiff_i(\tau), \qdiff_{\mi}(\tau))].
\end{align*}
Since for all $\i \in \I$, $\gibr(\theta, \qdiff_{\mi}(\tau)) \in \argmax_{\qdiff_i(\tau) \in \Qi} \mathbb{E}_{\theta}[\Psi^s(\qdiff_i(\tau), \qdiff_{\mi}(\tau))]$ and $\alpha_i>0$, we have:
\begin{align*}
 \frac{d \mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))]}{d \tau}  \left\{
\begin{array}{ll}
>0, & \quad \text{If $\qdiff(\tau) \notin \EQ(\theta)$}, \\
=0, & \quad \text{If $\qdiff(\tau) \in \EQ(\theta)$. }
\end{array}
\right.
\end{align*} 
That is, the value of the potential function $\mathbb{E}_{\theta}[\Psi^s(\tilde{q}(\tau))]$ strictly increases in $\tau$ except for $\tilde{q}(\tau)$ in the equilibrium set $\EQ(\theta)$. Since the value of the potential function is finite, we must have $\lim_{\tau \to \infty} \mathrm{dist}\( \tilde{q}(\tau), \EQ(\theta)\)=0$ for all $\theta \in \Delta(\S)$.
\QEDA 



\vspace{0.2cm}


\noindent\textbf{\emph{Proof of Proposition \ref{prop:supermodular}.}}

We first prove \emph{2}. For any $\i \in \I$ and any $\theta$, $\BRi(\theta, \q_{\mi}) = \argmax_{\qi \in \Qi} \mathbb{E}_{\theta}[u_i^s(\qi, \qmi)]$. Since $u_i^s(\qi, \qmi)$ is concave in $\qi$ for all $\s \in \S$, the function $\mathbb{E}_{\theta}[u_i^s(\qi, \qmi)]$ is also concave in $\qi$. Therefore, the set $\BRi(\theta, \qmi) $ must be an interval with the minimum best response strategy $\hmin_i(\theta, \q)$ and the maximum best-response strategy $\hmax_i(\theta, \q)$. Moreover, from Berge's maximum theorem, since $\mathbb{E}_{\theta}[u_i^s(\qi, \qmi)]$ is continuous in $\q$ and $\theta$, $\BRi(\theta, \qmi) $ is upper-hemicontinuous in $\qmi$ and $\theta$. 

Next, we prove \emph{1}. Consider the process of iterated deletion of strictly dominated strategy of game $G_D$ with belief $\theta$: In the first round, we delete the set of strategies of player $\i$ that are not a best response strategy for any $\qmi \in \Qmi$ in game $G_D$ with belief $\theta$. We denote the remaining strategies of each player $\i \in \I$ as $R^1_i(\theta)$. Then, any strategy $\qi \in R_i^1(\theta)$ must be a best response of at least one $\qmi \in \Qmi$, i.e. $R_i^1(\theta) = \cup_{\qmi \in \Qmi} \BRi(\theta, \qmi)$. From \emph{2}, we know that $\BRi(\theta, \qmi)$ is an interval in the set $\Qi$ for any $\qmi \in \Qmi$, and $\BRi(\theta, \qmi)$ is upper-hemicontinuous in both $\theta$ and $\qmi$. Therefore, the strategy set $R_i^1(\theta)$ is an interval in $\Qi$, and $R_i^1(\theta)$ is upper-hemicontinuous in $\theta$. We denote the set of player $\i$'s strategies that are not deleted after round $n \geq 1$ as $R^{n}_i(\theta)$. In step $n+1$, we delete the set of player $\i$'s strategies that are not a best response strategy for any $\qmi \in \prod_{j \in \I \setminus \{\i\}} R_i^{n}(\theta)$, and the set of remaining strategies is $R_i^{n+1}(\theta)$. Then, any strategy $\qi \in R_i^n(\theta)$ must be a best response of some opponents' strategy profile in $R_{\mi}^{n-1}(\theta) \deleq \prod_{j \in \I \setminus \{i\}} R_{j}^{n-1}(\theta)$, i.e. $R_i^n(\theta) = \cup_{\qmi \in R_{\mi}^{n-1}(\theta)} \BRi(\theta, \qmi)$.
Therefore, the strategy set $R_i^n(\theta)$ must be an interval in $\Qi$, and $R_i^n(\theta)$ is upper-hemicontinuous in $\theta$ for each round $n$. 

The process of iterated deletion of dominated strategies stops when no strategy can be deleted for any player. Since the game $G_D$ is a dominance solvable game, the rationalizable strategies $\R(\theta) = \prod_{\i \in \I} \R_i(\theta)$ is a singleton set that contains the unique equilibrium strategy profile $\gwe(\theta)$. Therefore, we can conclude that the rationalizable strategy set $R(\theta) = \{\gwe(\theta)\}$ is upper-hemicontinuous in $\theta$, which implies that the unique equilibrium strategy profile $\gwe(\theta)$ is continuous in $\theta$. 



Finally, we prove \emph{3}: To begin with, we can show that any solution $\qdiff(\tau)$ of the differential inclusion \eqref{eq:differential_inclusion} satisfies that for any $\i \in \I$, $\lim_{\t \to \infty} \mathrm{dist}\(\qdiff_i(\tau), R^1_i(\theta)\) =0$, where $ R^1_i(\theta)$ is the set of player $\i$'s strategies that survive the first round of deletion of strictly dominated strategies. For any $\i \in \I$, we consider the function $v^1_i(\tau)= \mathrm{dist}\(\qdiff_i(\tau), R^1_i(\theta)\) ^2$. From \emph{1}, we know that the set $R^1_i(\theta)$ is an interval in $\Q_i$. Therefore, we can write $R^1_i(\theta) = [\Rlow_i^1, \Rup_i^1]$, where $\Rlow_i^1$ (resp. $\Rup_i^1$) is the minimum (resp. maximum) strategy in the set $R^1_i(\theta)$. Therefore, 
\begin{align*}
v^1_i(\tau)= \left\{
\begin{array}{ll}
\(\qdiff_i(\tau) - \Rlow^1_i\)^2, & \quad \text{if $\qdiff_i(\tau) <\Rlow^1_i$},\\
0, & \quad \text{if $\qdiff_i(\tau) \in [\Rlow^1_i, \Rup^1_i]$},\\
\(\qdiff_i(\tau) - \Rup^1_i\)^2, & \quad \text{if $\qdiff_i(\tau) > \Rup^1_i$}. 
\end{array}
\right.
\end{align*}
Then, 
\begin{align*}
&\frac{d v_i^1(\tau)}{d \tau} = \frac{d v_i^1(\tau)}{d \qdiff_i(\tau)}\frac{d \qdiff_i(\tau)}{d \tau}\\
\stackrel{\eqref{eq:differential_inclusion}}{\in}&\left\{
\begin{array}{ll}
2 \alpha_i\(\qdiff_i(\tau) - \Rlow^1_i\) \(\BRi(\theta, \qdiff(\tau))-\qdiff_i(\tau)\), &  \quad \text{if $\qdiff_i(\tau) <\Rlow^1_i$},\\
0, & \quad \text{if $\qdiff_i(\tau) \in [\Rlow^1_i, \Rup^1_i]$},\\
2 \alpha_i\(\qdiff_i(\tau) - \Rup^1_i\)  \(\BRi(\theta, \qdiff(\tau))-\qdiff_i(\tau)\), &  \quad \text{if $\qdiff_i(\tau) >\Rup^1_i$},
\end{array}
\right.
\end{align*}
where $\alpha_i \in [\nu, 1]$. Since $\BRi(\theta, \qdiff(\tau)) \in [\Rlow^1_i, \Rup^1_i]$, we have 
\begin{align*}
\frac{d v^1_i(\tau)}{d \tau}  \leq -2 \alpha_i \mathrm{dist}\(\qdiff_i(\tau), R^1_i(\theta)\) ^2 = - 2 \alpha_i v^1_i(\tau) \left\{
\begin{array}{ll}
<0, &  \quad \text{if $\qdiff_i(\tau) <\Rlow^1_i$},\\
=0, & \quad \text{if $\qdiff_i(\tau) \in [\Rlow^1_i, \Rup^1_i]$},\\
<0, &  \quad \text{if $\qdiff_i(\tau) >\Rup^1_i$}.
\end{array}
\right.
\end{align*}
That is, as $\tau$ increases, the value of the function $v^1_i(\tau)$ strictly decreases so long as $\qdiff_i(\tau) \neq R_i^1(\theta)$. Since $v^1_i(\tau) \geq 0$, we must have $\lim_{\t \to \infty}  v^1_i(\tau) =0$ for all $\i \in \I$, i.e. $\lim_{\t \to \infty} \mathrm{dist}\(\qdiff_i(\tau), R^1_i(\theta)\) =0$ for all $\i \in \I$. 

Suppose that in $n$-th round, $\lim_{\t \to \infty} \mathrm{dist}\(\qdiff_i(\tau), R^n_i(\theta)\) =0$ for all $\i \in \I$. Following the same procedure as $n=1$, we can show that the set $R^{n+1}_{\i}$ is an interval $[\Rlow^{n+1}_i, \Rup^{n+1}_i]$, where $\Rlow^{n+1}_i$ (resp. $ \Rup^{n+1}_i$) is the smallest (resp. largest) strategy of player $\i$ after the $n+1$-th iteration. Then, by defining $v^{n+1}_i(\t)= \mathrm{dist}\(\qdiff_i(\tau), R^{n+1}_i(\theta)\) ^2$ for all $\i \in \I$, we can show that $\lim_{\t \to \infty}  v^{n+1}_i(\tau) =0$ and hence  $\lim_{\tau \to \infty} \mathrm{dist}\(\qdiff_i(\tau), R^{n+1}_i(\theta)\) =0$ for all $\i \in \I$. From mathematical induction, we can conclude that $\lim_{\tau \to \infty} \mathrm{dist}\(\qdiff_i(\tau), R_i^n(\theta)\) =0$ for all $\i \in \I$ and all $n\geq 1$. Therefore, $\lim_{\tau \to \infty} \mathrm{dist}\(\qdiff_i(\tau), R_i(\theta)\) =0$. Since $G_D$ is dominance-solvable, we must have $\lim_{\tau \to \infty} \qdiff_i(\tau)= \gwe_i(\theta)$. That is, any solution $\qdiff(\tau)$ of the differential inclusion \eqref{eq:differential_inclusion} converges to the unique equilibrium strategy profile $\gwe(\theta)$. 
\QEDA 

==> proof_stability_br.tex <==
% !TEX root = main041620.tex
%%novalidate
\noindent\emph{\textbf{Proof of Lemma \ref{lemma:residual_zero}}.} For any $\i \in \I$ and any $\t$, the residual term $\xi_i^\t = \gibr(\thetatone, \qt_{\mi}) - \tilde{h}_i(\thetabar, \qt_{\mi})$ is bounded because both $\gibr(\thetatone, \qt)$ and $\tilde{h}_i(\thetabar, \qt_{\mi})$ are feasible strategies of player $\i \in \I$ in the bounded set $\Qi$. Additionally, 
\begin{align*}&\|\xi_i^\t\| =  \|\gibr(\thetatone, \qt_{\mi}) - \tilde{h}_i(\thetabar, \qt_{\mi})\|\\
=& \left\|\gibr(\thetatone, \qt_{\mi})- \argmin_{\qi \in \BRi(\thetabar, \qt_{\mi})} |\qi-\gibr(\thetatone, \qt_{\mi})|\right\| 
=d\(\gibr(\thetatone, \qt_{\mi}), \BRi(\thetabar, \qt_{\mi})\). \end{align*} 

From Assumption \textbf{(A5)} and the fact that $\lim_{\t \to \infty} \thetat=\thetabar$, we know that for any $\delta>0$, we can find a positive integer $K$ such that for any $\t > K$, $\BRi(\thetatone, \qt_{\mi}) \subseteq N_{\delta}\(\BRi(\thetabar, \qt_{\mi})\)$. Since $\gibr(\thetatone, \qt_{\mi}) \in \BRi(\thetatone, \qt_{\mi})$, we must have $\lim_{\t \to \infty} d\(\gibr(\thetatone, \qt_{\mi}), \BRi(\thetabar, \qt_{\mi})\)=0$ with probability 1. Therefore, we can conclude that $\lim_{\t \to \infty}\xi_i^\t=0$ with probability 1. \QEDA


\vspace{0.2cm}

\noindent\textbf{\emph{Proof of Lemma \ref{lemma:consistency_br}.}} We prove that for any $\s \in \S \setminus \Sequiv(\limitq)$, $\thetabar(\s)=0$ with probability 1. In particular, we consider the following two cases:\\
\emph{(Case 1):} The sequence $\(\qt\)_{\t=1}^{\infty}$ converges to a fixed point strategy $\qbar$. \\
In this case, $\limitq=\{\qbar\}$ is a singleton set, and Lemma \ref{lemma:consistency} directly shows that $\thetabar(\s)=0$ for all $\s \in \S\setminus \Sequiv(\qbar)$. \\
\emph{(Case 2):} The sequence $\(\qt\)_{\t=1}^{\infty}$ does not converge.\\
In this case, for any $\s \in \S \setminus \Sequiv(\limitq)$, there must exist a strategy $\qbar^1 \in \limitq$ such that $\s \notin \Sequiv(\qbar^1)$ (Definition \ref{def:set_payoff}). From Definition \ref{def:limit_point}, we know that we can find a subsequence $\(\q^{\tk_1}\)_{j=1}^{\infty}$ that converges to $\qbar^1$. 



If $\phi^{\sran}(\cbar|\qbar^1)$ is absolutely continuous in $\phi^{\s}(\cbar|\qbar^1)$, then we further decompose the remaining strategies into converging subsequences. If the remaining strategies form a converging sequence, then we have decomposed $\(\qt\)_{\t=1}^{\infty}$ into two converging subsequences with two limit points $\{\qbar^1, \qbar^2\}$. Otherwise, we can repeat this process of finding converging subsequences until all strategies in $\(\qt\)_{\t=1}^{\infty}$ are assigned to a subsequence. The total number of subsequences is denoted as $M$. For any $m=1, \dots, M$, and any $\t$, we denote $\tau_m^\t$ as the number of strategies in $\(\qj\)_{j=1}^{\t}$ that belongs to the $m$-th subsequence. Therefore, we can write the log-likelihood ratio as follows: 
\begin{align}
&\lim_{\t\to \infty}\frac{1}{\t}\log \(\frac{\Phi^\s(Y^k|Q^k)}{\Phi^{\sran}(Y^k|Q^k)}\)=  \lim_{\t\to \infty}\frac{1}{\t} \sum_{\j=1}^{\t} \log\(\frac{\phibar^{\s}(\cj|\qj)}{\phibar^{\sran}(\cj|\qj)}\)\notag\\
=&\lim_{\t\to \infty}\frac{\tau_1^{\t}}{\t}\(\frac{1}{\tau_1^\t}\sum_{j=1}^{\tau_1^{\t}} \log\(\frac{\phibar^{\s}(\c^{\tk_1}|\q^{\tk_1})}{\phibar^{\sran}(\c^{\tk_1}|\q^{\tk_1})}\)\)+ \sum_{m=2}^{M}\frac{\tau_m^{\t}}{\t} \(\frac{1}{\tau_m^{\t}}\sum_{j=1}^{\tau_m^{\t}} \log\(\frac{\phibar^{\s}(\c^{\tk_m}|\q^{\tk_m})}{\phibar^{\sran}(\c^{\tk_m}|\q^{\tk_m})}\)\)\label{eq:vague}
\end{align}
Analogous to \eqref{eq:hold}, for each $m$, as the subsequence $\(\q^{\tk_m}\)_{j=1}^{\infty}$ converges to $\qbar_m$, we have: 
\begin{align*}
\lim_{\t \to \infty} \frac{1}{\tau_m^{\t}}\sum_{j=1}^{\tau_m^{\t}} \log\(\frac{\phibar^{\s}(\c^{\tk_m}|\q^{\tk_m})}{\phibar^{\sran}(\c^{\tk_m}|\q^{\tk_m})}\) \left\{
\begin{array}{ll}
<0, & \quad \text{if $\s \notin \Sequiv(\qbar_m)$,}\\
=0, & \quad \text{otherwise.}
\end{array}
\right.
\end{align*}
From the way we construct the subsequences, we know that $\s \notin \Sequiv(\qbar_1)$. Therefore, from \eqref{eq:vague} we have $\lim_{\t \to \infty} \log \(\frac{\Phi^\s(Y^k|Q^k)}{\Phi^{\sran}(Y^k|Q^k)}\)=-\infty$. Hence, analogous to the proof of Lemma \ref{lemma:consistency}, we know that $\lim_{\t \to \infty} \thetat(\s)=0$ with probability 1. Note that this procedure can be applied to any $\s \in \S \setminus \Sequiv(\limitq)$. Hence, we can conclude that $\lim_{\t \to \infty} \thetat(\s)=0$ for any $\s \in \S \setminus \Sequiv(\limitq)$ with probability 1.

Finally, consider the situation where $\phi^{\sran}(\cbar|\qbar^1)$ is not absolutely continuous in $\phi^{\s}(\cbar|\qbar^1)$. Analogous to the analysis in case 2 of Lemma \ref{lemma:consistency}, we can apply Borel-Cantalli lemma on this strategy subsequence to show that there exists a finite step $K>0$ such that $\thetat(\s)=0$ for any $\t>K$ with probability 1. Hence, $\lim_{\t\to \infty} \thetat(\s)=0$ with probability 1.\QEDA

\vspace{0.2cm}

\noindent\textbf{\emph{Proof of Theorem \ref{theorem:stability_br}.}}  For any $\loadepfin>$ and any $\thetaepfin>0$, we define $\deltahat \deleq \min\{\delta, \loadepfin\}$. From condition (b), we know that $[\thetabar] \subseteq \Sequiv(\q)$ for any $\q \in \Qhat$. From condition (a), we can find a positive number $\epsilon'$ such that if $\theta \in N_{\epsilon'}(\thetabar)$, then $\EQ(\theta) \subseteq \Qhat$. We define $ \epsilonhat \deleq \min\left\{\thetaepfin, \epsilon, \epsilon'\right\}$. Then, again from condition (b), $\BR(\theta, \q) \subseteq N_{\delta}\(\EQ(\thetabar)\)$ for any $\theta \in \Thetahat$ and any $\q \in N_{\delta}\(\EQ(\thetabar)\)$. %We can also check that $\EQ(\theta) \subseteq \Qhat$ for any $\theta \in \Thetahat$.  


Analogous to the proof of Lemma \ref{lemma:stopping_time}, we can show that if $\thetazero(\s)< \rhoone$ for all $\s \in \S \setminus [\thetabar]$ and $|\thetazero(\s)-\thetabar(\s)|<\rhoone$ for all $\s \in [\thetabar]$, then $\pro\(\thetat(\s)\leq \rhotwo, ~\forall \s \in \Sbar, ~ \forall \t\)>\gamma$. The thresholds $\rhoone$ and $\rhotwo$ are from \eqref{eq:rhoone} -- \eqref{eq:rhotwo}.  

Next, consider any $\q^1 \in N_{\delta}\(\EQ(\thetabar)\)$ and any $\thetazero$ that satisfies $|\thetazero(\s)- \thetabar(\s)|< \rhothree$ for all $\s \in [\thetabar]$. Since $[\thetabar] \subseteq \Sequiv(\q)$ for any $\q \in N_{\delta}\(\EQ(\thetabar)\)$, we have $[\thetabar] \subseteq \Sequiv(\q^1)$. Analogous to the proof of Lemma \ref{lemma:other_parameters}, we can show that if $|\thetazero(\s)-\thetabar(\s)|<\rhotwo$ for all $\s \in \Sbar$, then $\theta^2(\s) \in \(\thetabar(\s)-\frac{\epsilonhat}{|\S|}, \thetabar(\s)+\frac{\epsilonhat}{|\S|}\)$ for all $\s \in [\thetabar]$. Moreover, if $\theta^2(\s)<\rhotwo$ for all $\s \in \Sbar$, then $\theta^2 \in N_{\epsilonhat}\(\thetabar\)$. From condition (b), we know that $\BR(\theta^2, \q^1) \in N_{\delta}\(\EQ(\thetabar)\)$. Therefore, the updated strategy $\q^2 \in N_{\delta}\(\EQ(\thetabar)\)$. Condition (b) further ensures that $[\thetabar] \subseteq \Sequiv(\q^2)$. 

By using mathematical induction for $\t>2$, we have: 
\begin{align*}
\pro\(\left.\begin{array}{l}
|\thetat(\s)-\thetabar(\s)|<\frac{\epsilonhat}{|\S|}, ~\forall \s \in [\thetabar], ~\forall \t\\
\qt \in N_{\delta}\(\EQ(\thetabar)\), ~\forall \t
\end{array}\right\vert
\thetat(\s)<\rhotwo, ~\forall \s \in \Sbar, ~\forall \t\)=1.
\end{align*} 
Finally, for any $\gamma \in (0, 1)$, and any $\thetaepfin, \loadepfin >0$, we consider $\loadep =\delta$ and $\thetaep = \min\{\rhoone, \rhothree\}$. If $\thetazero \in N_{\epsilon^1}(\thetabar)$ and $\q^1 \in N_{\delta^1}\(\EQ(\thetabar)\)$, then
\begin{align*}
& \pro\(\thetat \in \Thetahat, ~  \qt \in N_{\delta}\(\EQ(\thetabar)\), ~ \forall \t\)
\geq \pro\(\begin{array}{l}
|\thetat(\s)-\thetabar(\s)|<\frac{\epsilonhat}{|\S|}, ~ \forall \s \in [\thetabar], \forall \t\\
\thetat < \rhotwo, \forall \s \in \Sbar,  \qt \in N_{\delta}\(\EQ(\thetabar)\), \forall \t
\end{array}\) \\
 =& \pro\(\thetat(\s)<\rhotwo, \forall \s \in \Sbar, \forall \t\) \\
 &\qquad \cdot \pro\(\left.\begin{array}{l}
|\thetat(\s)-\thetabar(\s)|<\frac{\epsilonhat}{|\S|}, \forall \s \in [\thetabar], \forall \t\\
 \qt \in N_{\delta}\(\EQ(\thetabar)\), \forall \t
\end{array}\right\vert
\thetat(\s)<\rhotwo, \forall \s \in \Sbar, \forall \t\)\\
=&\pro\(\thetat(\s)<\rhotwo, \forall \s \in \Sbar, \forall \t\)>\gamma.
\end{align*}
Furthermore, from Theorem \ref{prop:asynchronous}, if $\thetat \in \Thetahat$ for all $\t$, then $\lim_{\t \to \infty} \thetat \in \Thetahat \subseteq \neighinftheta(\thetabar)$, $\qt$ converges to the equilibrium set associated with a belief in $\Thetahat$. Since for any $\theta \in \Thetahat$, $\EQ(\theta) \subseteq \Qhat \subseteq N_{\loadepfin}(\EQ(\thetabar))$, $\qt$ must converge to the set $N_{\loadepfin}(\EQ(\thetabar))$. Therefore, 
\begin{align*}
\lim_{\t \to \infty} \pro\(\thetat \in \neighinftheta(\thetabar), ~ \qt \in \neighinfload(\EQ(\thetabar))\) \geq  \pro\(\thetat \in \Thetahat, ~  \qt \in N_{\delta}\(\EQ(\thetabar)\), ~ \forall \t\)> \gamma. 
\end{align*}
Thus, we can conclude that $\(\thetabar, \EQ(\thetabar)\)$ is locally stable. \QEDA 

   
\vspace{0.2cm}




